SAWL:A Self-adaptive Wear-leveling NVM Scheme for High Performance Storage Systems

In order to meet the needs of high performance computing (HPC) in terms of large memory, high throughput and energy savings, the non-volatile memory (NVM) has been widely studied due to its salient features of high density, near-zero standby power, byte-addressable and non-volatile properties. In HPC systems, the multi-level cell (MLC) technique is used to significantly increase device density and decrease the cost, which however leads to much weaker endurance than the single-level cell (SLC) counterpart. Although wear-leveling techniques can mitigate this weakness in MLC, the improvements upon MLC-based NVM become very limited due to not achieving uniform write distribution before some cells are really worn out. To address this problem, our paper proposes a self-adaptive wear-leveling (SAWL) scheme for MLC-based NVM. The idea behind SAWL is to dynamically tune the wear-leveling granularities and balance the writes across the cells of entire memory, thus achieving suitable tradeoff between the lifetime and cache hit rate. Moreover, to reduce the size of the address-mapping table, SAWL maintains a few recently-accessed mappings in a small on-chip cache. Experimental results demonstrate that SAWL significantly improves the NVM lifetime and the performance for HPC systems, compared with state-of-the-art schemes.

==> introduction.tex <==
\section{Introduction}
%\vspace{-0.2cm}
The rapid growth in the core count of many-core processors has enabled applications with large numbers of threads that demand a large-capacity memory system. The scalability of the existing DRAM technology has reached the limits of the CMOS fabrication technology ~\cite{wilson2013international}, beyond which more errors and reliability problems will ensue due to process variation. In the meantime, several studies \cite{lefurgy2003energy,memorypower} have shown that leakage energy grows with the memory capacity, dissipating as much heat as dynamic energy and is a large contributor to operational cost. {Hence,} non-volatile memory (NVM) technologies
\cite{chen2010advances,chen2003access,endoh2016overview,kultursay2013evaluating,lee2010phase}, such as STT-RAM, PCM, and RRAM, have been proposed to alleviate the large leakage energy and poor scalability problems of the traditional DRAM technology. NVM technologies have many salient features, such as low-cost, shock-resistance, non-volatility, high density and power-efficiency. PCM and RRAM are considered as viable alternatives for the design of main memory \cite{volos2011mnemosyne,wei2015accelerating} due to their high storage density and low access latency.


It is projected that the multi-level-cell (MLC) technique will be widely applied to NVM (PCM and RRAM), leading to their rapid growth in device capacity and density but at the cost of much weaker endurance than their single-level-cell (SLC) counterparts. The advanced fabrication technique packs more than one bit in a single cell \cite{lee2012multi}, thus allowing NVM to achieve ultra-high density for mass storage applications. However, due to the iterative program-and-verify (P\&V) technique, the MLC technology tends to have remarkable variations on access latency and cell endurance. Table \ref{table1} summarizes the characteristic parameters of SLC and MLC NVM technologies. 
Compared with SLC, the MLC NVM increases access latency by 2$\sim$4 times and decreases endurance by 100 times because of unavoidable over-programming operation. For example, the SLC PCM devices are expected to last for ${10}^{7}\sim{10}^{8}$ writes per cell \cite{freitas2008storage,zhao2014slc}, and the RRAM technology has a per-cell write limit of between ${10}^{8}$ and ${10}^{12}$ in the SLC mode. But the cell endurance of MLC PCM only reaches ${10}^{5}\sim{10}^{6}$ writes per cell~\cite{gleixner2009reliability}, and that of the MLC RRAM decreases to ${10}^{7}$ writes per cell \cite{lee2012multi}.
%More seriously, the future MLC technique that stores more bits in a single cell will further decrease the endurance.


\begin{table}[h]
%\vspace{-0.3cm}
\linespread{1.4}
\centering
\scriptsize
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{5pt}
\caption{Key features of SLC and MLC NVM technologies.}
\label{table1}
\begin{tabular}{|l|c|c|c|c|}
\hline
              & SLC PCM   & SLC RRAM & MLC PCM    & MLC RRAM \\ \hline
Read latency  & 150ns & 10ns   & 250ns      & 50ns    \\ \hline
Write latency & 450ns     & 50ns & 1.5us & 350ns    \\ \hline
Cell endurance     & $10^{7} \sim 10^{8}$   & $10^{8} \sim 10^{12}$ & $10^{5} \sim 10^{6}$    & $\sim$ $10^{7}$      \\ 
\hline
\end{tabular}
\label{table1}
\end{table}


%Although the MLC technology is attracting widespread attention, its poor endurance restricts its system lifetime, exposes security vulnerability, and hinders its practical use as main memory. In other words,
%{Due to the poor cell endurance, MLC NVM systems are facing the risk of security vulnerability under malicious codes and general} applications with non-uniform access patterns. For a 64GB NVM system with an endurance of ${10}^{6}$ writes per cell, while a program with a perfectly uniform-access pattern allows the baseline system to obtain almost ideal lifetime, e.g., a lifetime of 24.7 months when the write traffic is 1GBps (i.e., $\frac{NVM \ capacity \ \times \ Wmax}{write \ traffic \ per \ second}$, where $Wmax$ represents the endurance per line). However, the omnipresent non-uniform accesses in real-world workloads are shown to cause line failures of NVM devices in much earlier stages, e.g., even with significant amount of spare lines, the baseline system achieves an average lifetime of only 1.2 months (5\% of the ideal lifetime) \cite{qureshi2009enhancing}. To make things worse, it has been demonstrated that, when facing malicious attacks, some NVM lines can be worn out in just 10 seconds (e.g., $2\times(t_w + t_r)\times Wmax $) by simple buffer-overflow attacks \cite{seong2010security}. Therefore, NVM systems should be designed to survive worst-case applications and malicious attacks. In this paper, our work focuses on improving the lifetime and reducing the security vulnerability.

The wear-leveling technique attempts to make write operations uniformly distributed by frequently remapping logical lines to new physical positions, which can significantly extend the lifespan of an NVM system and prevent brute-force attack to a certain physical line. {However, we observe that existing wear-leveling algorithms \cite{qureshi2009enhancing,seong2010security,seznec2009towards,zhao2014slc,zhao2014leveling} initially designed for SLC NVM, lose effectiveness in MLC NVM systems. Specifically,} to prevent the malicious attacks~\cite{seong2010security} that guess the physical location and continuously wear a given line, existing algorithms perform the remapping in the randomized manner without recording the accurate write counts of each memory cells. Hence, they attempt to achieve wear leveling by randomly shuffling logical-physical address mappings via algebraic functions to evenly disperse the logical lines written most frequently to as many physical lines as possible. This requires a huge number of rounds of data exchanges before a probabilistically uniform distribution of write counts of all physical lines in an NVM can be achieved \cite{yu2012increasing,qureshi2011practical}. %Thus, to achieve a good balance of write counts among memory lines, data exchanges must be executed for a very large number of rounds.
However, in practice, the low endurance of MLC NVM implies that some cells can be worn out long before this uniform distribution is reached. {As a result,} existing work fails to attain long lifetime of MLC NVM (the quantitative analysis is shown in Section 2).


There are two straightforward solutions to accelerate data exchanges and avoid some lines being worn out before they have a chance to be swapped. One is to increase the exchange frequency. However, frequent content exchanges increase write amplification, which in turn {significantly} decrease performance and increase energy consumption.
%More seriously, even if the wear-leveling schemes swap data frequently, the lifetime of MLC NVM is still seriously deficient (as described in Section~2).
The other is to decrease the wear-leveling granularity (e.g., \emph{region size}) to mitigate the imbalanced writes across the entire memory, which however significantly increases the size of address mapping table (e.g., hundreds of megabytes). Consequently, the mapping table is so large that it must be held on the NVM devices as opposed to SRAM in the memory controller, leading to severe performance degradation due to the very long address translation latency.
%Their severe performance degradation is unacceptable for many real-world applications.

{To address this problem, we consider} a tiered architecture which stores the entire address mapping table in the main memory (DRAM or NVM devices) and holds the recently-accessed entries in a small on-chip SRAM cache. {However, this naive architecture} often fails to provide sufficient performance improvement under the applications with substantial random access patterns because of the very low cache hit rate of such applications. {Hence,} we propose a self-adaptive wear-leveling scheme (SAWL) that dynamically changes the wear-leveling granularity to accommodate more useful addresses in the cache, thus improving cache hit rate significantly. {As a result,} SAWL is able to achieve both long lifetime and high performance. The main contributions of this paper can be summarized as follows:

\begin{enumerate}
  \item {\emph{\textbf{Insights for wear-leveling schemes on MLC NVM.}} We investigate the effectiveness that state-of-the-art wear-leveling algorithms work on MLC NVM, including table-based wear-leveling (TBWL)~\cite{zhou2009durable}, algebraic-based wear-leveling (AWL)~\cite{qureshi2009enhancing,seong2010security}, and hybrid wear-leveling (HWL) schemes~\cite{seznec2009towards,yu2012increasing}. We observe that TBWL and AWL have the vulnerability of either Repeated Address Attack (RAA) or significant NVM lifetime reduction. HWL has the potential of achieving high lifetime but causes significant on-chip storage overhead to store address mappings.}
  \item {\emph{\textbf{An efficient wear-leveling scheme for MLC NVM.}} We propose a Self-Adaptive Wear-Leveling (SAWL) scheme for MLC NVM. SAWL maintains recently-accessed address mappings in a small on-chip cache managed by the memory controller. To improve the cache hit rate, SAWL dynamically changes the wear-leveling granularity by means of region-merge and region-split operations. As a result, SAWL is able to achieve both high lifetime and performance.}
  \item {\emph{\textbf{Implementation and evaluation.}} We have implemented SAWL and evaluated it using the gem5 simulator~\cite{binkert2011gem5}. Experimental results show that SAWL improves $25\%\sim51\%$ ($50\%\sim78\%$) of ideal lifetime for the MLC NVM system with ${10}^{6}$ (${10}^{5}$) cell endurance, compared with state-of-the-art wear-leveling algorithms. Moreover, existing wear-leveling schemes incur 25\% IPC decrease on average, while SAWL only decreases the IPC performance by 5\% on average, in comparison with a baseline system without any wear-leveling algorithm.}
\end{enumerate}

%First, to prolong MLC NVM lifetime and thus improve the reliability and robustness of main memory, we propose a tiered architecture for the wear-leveling algorithm, which stores the complete mapping table on the DRAM and NVM devices and maintains recently-used entries in a small-sized SRAM cache in the memory controller. This enables the wear-leveling algorithm to deploy a large number of regions to substantially reduce the wear-leveling granularity, which significantly increases the lifetime of MLC NVM systems due to the sufficient number of data exchanges within and among the regions.

%We evaluate SAWL on Gem5 simulator \cite{binkert2011gem5}. The experimental results show that, compared with the state-of-the-art wear-leveling algorithms (e.g., PCM-S with 1MB cache, the best lifetime of a 64GB MLC NVM system achieves 16.7 months (67\% of the ideal) with Wmax=${10}^{6}$ or 24 days (32\% of the ideal) with Wmax=${10}^{5}$ under the BPA), our algorithm enhances the lifetimes of MLC NVM to 23.4 months (93.7\% of the ideal) and 66.7 days (89\% of the ideal) with Wmax = ${10}^{6}$/${10}^{5}$ respectively. In addition, SAWL improves the lifetime of MLC NVM system with ${10}^{5}$ endurance to 92.5\% (on average) under general applications. What's more, our SAWL only decreases the IPC performance by 5\% on average in comparison with the fundamental system without any wear-leveling algorithm.







The rest of the paper is organized as follows. Section 2 introduces the background and motivation. The overall design of SAWL is described in Section 3. Section 4 presents the evaluation results and analysis. Section 5 reviews the related work. We conclude the paper in Section 6.

